Field theory and the physics of disordered systems

In this talk I will present some of the main difficulties we encounter in studying the large scale behavior of disordered systems. This presentation will be done using a field theory language. The difficulties in applying the standard renormalization group approach are due to the presence of strong non-perturbative effects that we do not know how to master. These difficulties are particular acute in the case of ferromagnets in random field, localized electrons, growth models and spin glasses. I will review the situation presenting at the end a promising approach based on fat diagrams.

==> rubinstein.ref.tex <==

\begin{thebibliography}{99}






 

\bibitem{RINO} K.G. Wilson, Phys. Rev. B {\bf 4}, 3184 (1971). K. G. Wilson and, J. Kogut, Physics Reports {\bf 12} , 75 (1974). G.Parisi, {\sl Field Theory, Disorder and Simulations}, World Scientific, (Singapore 1992).  J. Zinn-Justin,{\sl  Quantum Field Theory and Critical Phenomena} (Oxford University Press, Oxford, UK,
2002). D.J. Amit and V. Martin-Mayor, {\sl Field Theory, the Renormalization Group and Critical Phenomena} (World
Scientific, Singapore, 2005). G. Parisi, J. Stat. Phys. {\bf 23}, 49 (1980).


  
 \bibitem{Aging} L.C.E. Struik, Physical aging in amorphous polymers and other materials, (Elsevier, Amsterdam 1978), E. Vincent, V. Dupuis, M. Alba, J. Hammann and J.-P. Bouchaud, Europhys. Lett. {\bf 50}, 674 (2000).

 \bibitem{37} K. Jonason, E. Vincent, J. Hammann, J.-P. Bouchaud and P. Nordblad, Phys. Rev. Lett. {\bf 81}, 3243 (1998).
 \bibitem{38} L.F. Cugliandolo and J. Kurchan, Phys. Rev. Lett.  {\bf 71}, 173 (1993).
 D. H\`erisson and M. Ocio, Phys. Rev. Lett.  {\bf 88}, 257202 (2002).
 \bibitem{40} S.F. Edwards and P.W. Anderson, J. Phys. F  {\bf 5}, 965 (1975). K. Binder and A.P. Young, Rev. Mod. Phys.  {\bf 58}, 801 (1986).
 \bibitem{41} E. Vincent and J. Hammann, J. Phys. C  {\bf 20}, 2659 (1987).
 \bibitem{42} L.F. Cugliandolo and J. Kurchan, J. Phys. A  {\bf 27}, 5749 (1994). S. Franz, M. MŽzard, G. Parisi and L.
Peliti, Phys. Rev. Lett.  {\bf 81}, 1758 (1998).
  \bibitem{MPV} M\'ezard, M., Parisi, G.  and Virasoro, M.A.\emph{ Spin Glass Theory and Beyond}, World 
Scientific, Singapore, 1987.
\bibitem{65} G. Parisi and N. Sourlas, Phys. Rev. Lett. {\bf 43},
  744 (1979); G. Parisi, {\em An introduction to the statistical mechanics of amorphous system} in {\em Les Houches SessionXXXIX}, eds. J.B. Zuber and R. Stora (North-
Holland, Amsterdam, 1984).
\bibitem{84} G. Parisi, J. Phys. A  {\bf 14}, 735 (1981).
\bibitem{83} F. Wegner, Zeitschrift  f\"ur Physick B  {\bf 35}, 207 (1979).

\bibitem{LOC} F. Evers and A.D. Mirlin, Phys. Rev. Lett. {\bf  84}, 3690 (2000). A.D. Mirlin, Physics Reports  {\bf 326}, 259
(2000).
\bibitem{54} A.Vaknin, Z. Ovadyahu and M. Pollak, Phys. Rev. Lett. 84, 3402 (2000); Z Ovadyahu, Slow conductance relaxations; Distinguishing the Electron Glass from extrinsic
mechanisms, Arxiv preprint arXiv:0811.1899 (2008).
\bibitem{56} A. Amir, Y. Oreg and Y. Imry, A New Universality Class of Aging in Glassy Systems, preprint
arXiv:0902.1501.
\bibitem{57} C. De Dominicis, I. Kondor and T. Temesvari, in Spin Glasses and Random Fields,edited by A.P. Young
(World Scientific, Singapore, 1997); Eur. Phys. J. B 11, 629 (1999); T. Temesvari, I. Kondor and C. De Dominicis, Eur. Phys. J. B  {\bf 18}, 493 (2000).
\bibitem{DDG}C. De Dominicis and I. Giardina {\sl Random Fields and Spin Glasses: A Field Theory Approach}, Cambridge University Press (2006)

\bibitem{59} S. Franz, G Parisi and M.A. Virasoro, J. Phys. France  {\bf 4}, 1657 (1994).
\bibitem{60} S. Boettcher, Phys. Rev. Lett.  {\bf 95}, 197205 (2005).
\bibitem{63}  M. M\'ezard and G. Parisi, Eur.Phys. J. B  {\bf }20, 217 (2001).
\bibitem{69} M. Kardar, G. Parisi and Y.C. Zhang, Phys. Rev. Lett.  {\bf 56}, 889 (1986).
\bibitem{70}  L. Canet and M.A. Moore, Phys. Rev.
Lett.  {\bf 98}, 200602 (2007).
\bibitem{72} E. Marinari, A. Pagnani, G. Parisi and Z. Racz, Phys. Rev. E  {\bf 65}, 026136 (2002).
\bibitem{73} R.C. Ball and T.A. Witten, Phys. Rev. A  {\bf 29}, 2966 (1984).
\bibitem{DOT} V.S. Dotsenko, J. Stat. Mech. P06003 (2006); J. Stat. Mech. P09005 (2007)

\bibitem{FP} M.E. Ferrero and G. Parisi, J. Phys. A {\bf 29}, 3795 (1996).

\bibitem{E} K.B. Efetov, Physica A, 1 {\bf 67}, 119 (1990).
\bibitem{PSL} G. Parisi and F. Slanina, J. Stat. Mech. L02003 (2006).
\bibitem{VS} V. Sacksteder, Phys. Rev. D {\bf 76}, 105032 (2007)

 \end{thebibliography}


